A Sensory Feedback Control Law for Octopus Arm Movements

The main contribution of this paper is a novel sensory feedback control law for an octopus arm. The control law is inspired by, and helps integrate, several observations made by biologists. The proposed control law is distinct from prior work which has mainly focused on open-loop control strategies. Several analytical results are described including characterization of the equilibrium and its stability analysis. Numerical simulations demonstrate life-like motion of the soft octopus arm, qualitatively matching behavioral experiments. Quantitative comparison with bend propagation experiments helps provide the first explanation of such canonical motion using a sensory feedback control law. Several remarks are included that help draw parallels with natural pursuit strategies such as motion camouflage or classical pursuit.

==> arXiv submission/definitions.tex <==
%general
\def\R{{\mathds{R}}}
\def\C{{\mathds{C}}}
\def\N{{\mathds{N}}}
\def\Z{{\mathds{Z}}}
\def\Q{{\mathds{Q}}}
\def\0{{\mathbb{0}}}
\def\1{{\mathds{1}}}
%\def\I{{\mathds{I}}}
\def\T{{\mathds{T}}}
\def\Field{{\bf F}}
\def\H{{\mathcal H}}   % Used for the (true) Hamiltonian function
\def\U{{\mathcal U}}
\def\B{{\mathcal B}}
\def\A{{\mathcal A}}
\def\L{{\mathcal L}}
\def\g{{\mathfrak g}}
\def\tr{{\text{tr}}}


\def\r{{\mathbf{r}}}
\def\d{{\mathbf{d}}}

\def\a{{\mathbf{a}}}
\def\b{{\mathbf{b}}}

\def\m{{\bm{m}}}
\def\n{{\bm{n}}}
\def\f{{\bm{f}}}
\def\l{{\bm{l}}}

\def\Vecm {{\underline{\bm{m}}}}
\def\Vecn {{\underline{\bm{n}}}}
\def\Veckappa {{\underline{\bm{\kappa}}}}
\def\Vecnu {{\underline{\bm{\nu}}}}


\def\i{{\mathbf{i}}}
\def\j{{\mathbf{j}}}

\def\k{\kappa}


%\newcommand{\sobolev}{\mathbf{H}}


\def\maximize{\mathop{\rm maximize}}	
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\abs}[1]{\left| #1 \right|}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
%\renewcommand{\qedsymbol}{$\blacksquare$}

\definecolor{db}{RGB}{23,20,119}
\definecolor{dg}{RGB}{2,101,15}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
%\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}[section]

%specific to the document

\usepackage{upgreek}
\newcommand{\dif}{\mathrm{d}}
\newcommand{\transpose}{\intercal}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\defined}{\coloneqq}
\newcommand{\define}{\eqqcolon}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\euclideans}{\mathbb{E}}
\newcommand{\rotation}[1]{\mathrm{R}\left(#1\right)}
\newcommand{\rotationT}[1]{\mathrm{R}^\transpose\left(#1\right)}
\newcommand{\lab}[1]{#1}
\newcommand{\labv}[1]{\boldsymbol{\lab{#1}}}
\newcommand{\labm}[1]{\mathbf{#1}}
\newcommand{\material}[1]{
	\ifthenelse{\equal{#1}{\kappa}}{\upkappa}{
	\ifthenelse{\equal{#1}{\nu}}{\upnu}{
	\ifthenelse{\equal{#1}{\omega}}{\upomega}{
	\ifthenelse{\equal{#1}{\sigma}}{\upsigma}{
	\ifthenelse{\equal{#1}{\theta}}{\uptheta}{
	\mathsf{#1}}}}}}
}
\newcommand{\materialv}[1]{\boldsymbol{\material{#1}}}
\newcommand{\materialm}[1]{\boldsymbol{\material{#1}}}
\newcommand{\rowvector}[3]{\left[#1\ #2\ #3\right]^\transpose}
\newcommand{\colvector}[3]{\begin{bmatrix}#1\\#2\\#3\end{bmatrix}}


\newcommand{\target}{\text{target}}
\newcommand{\intrinsic}{\circ}
\newcommand{\head}{\text{h}}
\newcommand{\arm}{\text{arm}}
\newcommand{\deformations}{w}
\newcommand{\states}{q}
\newcommand{\momentums}{p}
\newcommand{\costates}{\xi}
\newcommand{\Hamiltonian}{\mathcal{H}}
\newcommand{\Lagrangian}{\mathcal{L}}
\newcommand{\potential}{\mathcal{V}}
\newcommand{\kinetic}{\mathcal{T}}
\newcommand{\mass}{M}
\newcommand{\controlHamiltonian}{H}
\newcommand{\ubar}{\b}
\renewcommand{\a}{\mathsf{a}}
\renewcommand{\b}{\mathsf{b}}
\newcommand{\ball}{\text{o}}



\newcommand{\muscle}{\text{m}}
\newcommand{\longitudinalmuscle}{\text{LM}}
\newcommand{\transversemuscle}{\text{TM}}
\newcommand{\Gmuscle}{\mathsf{G}}
\newcommand{\Rmuscle}{\mathsf{R}}
\newcommand{\rigid}{\zeta}
\newcommand{\rigidity}{\mathrm{r}}


%notation for spaces
\newcommand{\sobolev}{\mathrm{H}}
\newcommand{\lspace}{\mathrm{L}^2}
\newcommand{\controlspace}{\mathrm{U}}
\newcommand{\statespace}{\mathrm{Z}}




%Tixian's symbols
\newcommand{\ud}{\,\mathrm{d}}
\newcommand{\diag}{\text{diag}}
\newcommand{\uf}{u^F}
\newcommand{\uc}{u^C}
%\newcommand{\D}{\mathcal{D}^{\small{+}}}
%\newcommand{\diff}{\mathcal{D}^{\tiny{-}}}
\newcommand{\D}{\tilde{\mathcal{D}}}
\newcommand{\diff}{\bar{\mathcal{D}}}
\newcommand{\Ve}{\mathcal{V}^e}
\newcommand{\Vm}{\mathcal{V}^\text{m}}
\newcommand{\Vr}{\mathcal{V}^{\mathrm{r}}}
\newcommand{\LMt}{\mathrm{LM}_t}
\newcommand{\LMb}{\mathrm{LM}_b}
\newcommand{\TM}{\mathrm{TM}}
\newcommand{\LM}{\mathrm{LM}}
\newcommand{\range}{\Big|_{\sigma=0}^s}
\newcommand{\DDl}{\mathcal{D}^\text{linear}}
\newcommand{\DDd}{\mathcal{D}^\text{drag}}
\newcommand{\Dl}{D^\text{linear}}
\newcommand{\Dd}{D^\text{drag}}
\newcommand{\myper}{_\text{per}}
\newcommand{\mytan}{_\text{tan}}
\newcommand{\drag}{ f^\text{drag}}
\newcommand{\rhow}{\rho_\text{water}}
\newcommand{\qr}{\bar{q}}
\newcommand{\pr}{\bar{p}}
\newcommand{\Rho}{\mathrm{P}}
%\newcommand{\Rho}{\varrho}
\newcommand{\Angle}{\Theta}
\newcommand{\Htotal}{\mathcal{H}^\text{total}}
\newcommand{\radius}{\gamma^\text{rod}}
\newcommand{\rodtip}{\gamma^\text{tip}}
\newcommand{\rodbase}{\gamma^\text{base}}
\newcommand{\eff }{\text{eff}}
\newcommand{\dist}{\rho}
\newcommand{\distvec}{\boldsymbol\rho}
%\newcommand{\distvec}{{\sigma}^{\text{target}}}
\newcommand{\vel}{\boldsymbol v}
\newcommand{\unicycle}[1]{\mathsf{#1}}
\newcommand{\thetaUnicycle}{\vartheta}
\newcommand{\slope}{\mathsf{m}}
